An Efficient Distributed Multi-Agent Reinforcement Learning for EV Charging Network Control

The increasing trend in adopting electric vehicles (EVs) will significantly impact the residential electricity demand, which results in an increased risk of transformer overload in the distribution grid. To mitigate such risks, there are urgent needs to develop effective EV charging controllers. Currently, the majority of the EV charge controllers are based on a centralized approach for managing individual EVs or a group of EVs. In this paper, we introduce a decentralized Multi-agent Reinforcement Learning (MARL) charging framework that prioritizes the preservation of privacy for EV owners. We employ the Centralized Training Decentralized Execution-Deep Deterministic Policy Gradient (CTDE-DDPG) scheme, which provides valuable information to users during training while maintaining privacy during execution. Our results demonstrate that the CTDE framework improves the performance of the charging network by reducing the network costs. Moreover, we show that the Peak-to-Average Ratio (PAR) of the total demand is reduced, which, in turn, reduces the risk of transformer overload during the peak hours.

==> Conference_paper/Chapters/Introduction_Version1.tex <==
\section{Introduction}

In light of the growing concern surrounding climate change, Electric Vehicles (EVs) are increasingly seen as a promising solution to combat air pollution and global warming. As the EV penetration increases, the distribution grid faces considerable challenges. One prominent issue arises from the absence of coordination in EV charging, which has the potential to disrupt the normal pattern of residential electricity demand.

Charging control aims to effectively manage and coordinate the charging and discharging behavior of EVs to achieve various objectives. These objectives include minimizing charging costs for EV owners, meeting the user's battery energy requirements, reducing grid stress by balancing charging demand, and enhancing overall system efficiency. EV charging control seeks to provide users with a smooth and reliable charging experience while maximizing the benefits for both individuals and the grid. However, there are several challenges associated with EV charging control, including uncertainties in user behavior, scalability and congestion management of EVs, dynamic electricity prices, and accommodating user preferences and constraints. These challenges make it complex to derive an optimal charging strategy solely through analytical solutions using mathematical methods.

Researchers have developed many approaches to coordinate the charging process of EVs to avoid the transformer overload. These approaches can basically be categorized into two groups based on their model assumption: model-based and model-free methods. model-based approaches such as binary optimization~\cite{sun2016optimal}, mixed-integer linear programming~\cite{paterakis2016coordinated}, robust optimization~\cite{ortega2014optimal}, stochastic optimization~\cite{wu2017two}, model predictive control~\cite{zheng2018online}, and dynamic programming~\cite{xu2016dynamic} have been used for EV charging control and optimal scheduling considering electricity price uncertainty and users behavior. The challenges with these kinds of methods is that the EV charging scheduling problem is generally formulated as an optimization control problem with a known system transition function, which requires an accurate model or the forecasted results on the uncertainties.

In contrast, the model-free approaches do not require an accurate model or prior knowledge of the environment. Deep Reinforcement Learning (DRL) has demonstrated its great potential in sequential decision-making problems. DRL enables direct learning of optimal charging control behavior through interaction with the environment. Previous studies have utilized single-agent DRL techniques like Deep Deterministic Policy Gradient (DDPG) and Soft-Actor-Critic (SAC) for an individual EV or a group of EVs charging control and scheduling. These studies operate under the assumption of full observability of the environment. This means that the DRL agent should have access to the local information of the EVs, such as their online consumption, arrival/departure time and their battery level. However, the EV owners may be unwilling to share these personal information with other owners. To address this issue, as an extension of single-agent RL, Multi-Agent RL (MARL), which has been known as a powerful tool for distributed control, can be used for solving the EV network charging control problem.

In this paper, we model the charging control of an EVs network in residential sector. Our method utilizes a Partially Observable Markov Decision Process (POMDP) framework and incorporates a cutting-edge cooperative reinforcement learning technique called Multi-Agent Deep Deterministic Policy (MADDPG)~\cite{lowe2017multi}. Unlike previous works, we depart from the assumption of sharing global or local information among agents during execution. Instead, we adopt a centralized training-decentralized execution (CTDE) architecture that allows policies to leverage additional information for training purposes only, while still maintaining decentralized operation during execution. The only observation shared among agents in our framework is the electricity price. Once training is completed, only local actors are utilized during the execution phase, enabling effective and decentralized control that is applicable in cooperative settings. The main contributions of this article are as follows:

\begin{itemize}
    \item This paper presents a cooperative MARL framework for EVs network charging problem. We propose the mathematical analytics for distributed control, and the problem is formulated as POMDP. 
    \item We leverage the benefits of Centralized training decentralized execution framework to relax the assumption of observing the global network parameters and exchanging private information between agents.
    \item We examine the performance of our CTDE-oriented framework for a EV network. We provide the simulation results for up-to 10 agents and investigate the scalability of the proposed framework. 
\end{itemize}
The rest of this paper is organized as follows. Section~\ref{LitReview} provides the most recent related work. The network and system model formulation are described in Section~\ref{Background}. Section~\ref{Algorithm} introduced the proposed CTDE algorithm as well as the pricing scheme. Numerical results are presented in Section~\ref{results} and Section~\ref{conclusion} concludes the paper.


==> Conference_paper/Chapters/Introduction_Version2.tex <==
\section{Introduction}

As the number of Electric Vehicles (EVs) continues to increase, there is an increasing need for effective management and coordination of their charging and discharging behavior. This is where EV charging controls become essential. The objective of EV charging control is to ensure a smooth and reliable charging experience while maximizing the benefits for both individual EV owners and the overall grid network. In terms of individual benefits, EV charging control aims to minimize charging costs for owners and meet their battery energy requirements, which has been extensively researched~\cite{al2019review, abdullah2021reinforcement}. Additionally, for the grid network, charging control seeks to balance charging demand and prevent transformer overload during peak demand hours, which still remains an area under investigation~\cite{nimalsiri2019survey}. 

However, designing an optimal charging strategy for a network of EVs is a complex task due to several challenges. One of the primary challenges is the uncertainty in dynamic electricity prices, which is currently one of the most intriguing areas of focus in the field of smart grid technologies. Dynamic pricing can result in price fluctuations, making it difficult for EV owners to accurately predict the cost of charging their vehicles. Another challenge arises from the EV owners' behavior, which can vary widely. The arrival and departure times of EVs to the charging network do not follow a specific distribution, and EV owners may have different preferences regarding their desired charging level and preferred charging time. However, one of the most crucial challenges in an EV network is congestion management and transformer overload, which is the main focus of this paper. Simultaneous charging EVs have the potential to overwhelm the transformers connected to the network, and an optimal charging strategy should effectively manage this congestion. In this case, coordination and communication between the EVs can control and adjust their charging behavior based on real-time grid conditions. 

Considering the aforementioned challenges, for avoiding transformer overload, researchers have developed many approaches to coordinate the charging process of EVs network. These approaches can basically be categorized into two groups based on their model assumption: model-based and model-free methods. Model-based approaches such as binary optimization~\cite{sun2016optimal}, mixed-integer linear programming~\cite{paterakis2016coordinated}, robust optimization~\cite{ortega2014optimal}, stochastic optimization~\cite{wu2017two}, model predictive control~\cite{zheng2018online}, and dynamic programming~\cite{xu2016dynamic} have been used for EV charging control and optimal scheduling considering electricity price uncertainty and users behavior.  In these approaches, the scheduling of EV charging is typically framed as an optimization control problem, assuming a well-defined system transition function. This necessitates either a precise model or reliable forecasts. However, the challenges associated with these approaches arise from the difficulty of obtaining such precise models, especially in the presence of uncertainties.

In contrast, the model-free approaches offer an alternative that does not require an accurate model or prior knowledge of the environment.  Among these approaches, Deep Reinforcement Learning (DRL) stands out as a powerful technique for addressing sequential decision-making problems. In EV network, DRL allows for direct learning of optimal charging control behavior through interaction with the environment. Previous studies have utilized single-agent DRL techniques like Deep Deterministic Policy Gradient (DDPG) and Soft-Actor-Critic (SAC) for an individual EV or a group of EVs network, in which a single RL agent controls the charging power and charging scheduling of EVs during the charging phase. These studies operate under the assumption of full observability of the environment. This means that the DRL agent should have access to the local information of the EVs, such as their online consumption, arrival/departure time and their battery level. However, the EV owners may be unwilling to share these personal information with other owners. To tackle this concern, Multi-Agent RL (MARL) can be employed as an extension of single-agent RL. MARL is a powerful tool for distributed control, offering effective solutions to issues such as transformer overload and charging power control within EV networks.

In this paper, we model the charging control of an EVs network in residential sector. Our method utilizes a Partially Observable Markov Decision Process (POMDP) framework and incorporates a cutting-edge cooperative reinforcement learning technique called Multi-Agent Deep Deterministic Policy (MADDPG)~\cite{lowe2017multi}. Unlike previous works, we depart from the assumption of sharing global or local information among agents during execution. Instead, we adopt a centralized training-decentralized execution (CTDE) architecture that allows policies to leverage additional information for training purposes only, while still maintaining decentralized operation during execution. The only observation shared among agents in our framework is the electricity price. Once training is completed, only local actors are utilized during the execution phase, enabling effective and decentralized control that is applicable in cooperative settings. The main contributions of this article are as follows:

\begin{itemize}
    \item This paper presents a cooperative MARL framework for EVs network charging problem. The problem is formulated as POMDP, and the mathematical formulation for decentralized control has been proposed.
    \item We leverage the benefits of Centralized training decentralized execution framework to relax the assumption of observing the global network parameters and exchanging private information between agents.
    \item We examine the performance of our CTDE-oriented framework for a EV network. We provide the simulation results for up-to 10 agents and investigate the scalability of the proposed framework. 
\end{itemize}
The rest of this paper is organized as follows. Section~\ref{LitReview} provides the most recent related work. The network and system model formulation are described in Section~\ref{Background}. Section~\ref{Algorithm} introduced the proposed CTDE algorithm as well as the pricing scheme. Numerical results are presented in Section~\ref{results} and Section~\ref{conclusion} concludes the paper.


==> Conference_paper/Chapters/System_model1.tex <==

\section{Background}\label{Background}

\subsection{Demand-side Network}

Demand-side management (DSM) is a strategy used by utilities and grid operators to manage the demand for electricity during periods of peak usage. The primary goal of DSM is to reduce the overall demand for electricity by incentivizing consumers to shift their usage to non-peak hours or to reduce their overall consumption. In most of the traditional DSM programs, the interaction between utility company and end-users has been investigated, where each user individually respond to the program. Effective DSM programs have the potential to reduce the network demand and promote more sustainable energy usage. A good DSM program should have the objective that aggregate demand satisfies some desired properties and also meet the needs and expectations of end-users. For example, for solving the economic dispatch only the network demand is important and Peak-to-Average (PAR) depends only on the network demand. 
In this paper, we argue that such effective programs are not accessible unless the end-users actively particulate to the program and cooperate with each other. It is difficult to ensure the effective design of DSM programs with the aforementioned objectives without information exchange between end-users. How can the network objective be achieved when end-users are interacting within the environment on an individual basis?

The increasing adoption of EVs presents both opportunities and challenges for DSM initiatives. While EVs can help reduce the overall carbon footprint of transportation and contribute to a more sustainable energy system, they pose significant challenges, such as increasing the energy demand during peak periods. Consider, if numerous EVs are charging simultaneously during peak demand periods, it can place a strain on the energy grid and lead to blackouts. 

This paper presents a framework that automates energy management for an EVs network on the demand-side, which can be utilized in DSM programs. The scenario we consider involves multiple end-users who share a common energy source, such as a generator or substation transformer connected to the grid. Each user is equipped with an energy consumption scheduler (ECS) installed in their smart meter. The smart meters interact automatically using a distributed algorithm to determine the optimal energy consumption for EVs. The optimization objective is to reduce the energy cost of the EV network while also minimizing the network PAR. The primary aim of the network participants is to collaborate with each other to achieve the network's goals. It can also be seen that a pricing mechanism can provide the users with the incentives to cooperate. The price signal is the only information signal that broadcast to the end-users, and the users' aggregated demand is the only information signal send back to the utility company. 
\begin{figure}[!t]
   \centering
    \includegraphics[scale=0.67, trim = 0.2cm 0.2cm 0.2cm 0.2cm, clip]{Conference paper/figs/system model.png}
    \caption{System model}
    \label{System Model}
    \vspace{-.1in}
\end{figure}

\subsection{System Model}
A block diagram of demand-side electric power distribution is shown in Figure~\ref{System Model}. We assume that all the end-users are EV owners and are equipped with a smart meter and EV charging controller. The smart meters are all connected to the power line coming from the shared energy source, and they are also connected to each other through a communication channel. 

We model the distribution network in figure~\ref{System Model} as a graph $\mathcal{G} = (\mathscr{V},\mathscr{E})$, where $\mathscr{V} = \{0,1,...,N\}$ and $\mathscr{E} = \{1,2,...,M\}$ represent the set of nodes (users) and edges (branches), respectively. Node zero is considered as the connection to the shared energy source. For each user $i \in \mathscr{V}$, let $l_i^{h}$ denotes the total consumption of node $i$ at time $h$, where $h \in \mathcal{H} = \delequal \{1,..., \mathscr{H}\}$. $\mathscr{H}$ denotes the end time of charging period. Based on these definitions, $L_h = \sum\limits_{i \in \mathscr{V}}{l_i^h}$ represents the network total consumption at time $h$. For each user, let $\mathcal{X}_i$ denote the set of user appliances. Thus, the total consumption of the $i^{th}$ user is obtained as follows:
\begin{equation}
    l_i^h = \sum\limits_{a \in \mathcal{X}_i}{x_{i,a}^h} = \sum\limits_{a \in \mathcal{X}_i \char`\\\{EV\}}{x_{i,a}^h} + x_{i,EV}^h
\end{equation}
where $x_{i,a}^h$ denotes the consumption of the appliance $a$ of the user $i$ at time $h$.
The focus of this paper is EV charging control. Thus, without lack of generality, we assume that the total consumption of each user excluding the EV is constant. Thus, hereinafter, by $l_i^h$ we mean $x_{i,EV}^h$.






% The charging period peak and average also define as $L_{peak}= \max_{h \in \mathcal{H}}{L_h}$ and $L_{avg}=\frac{1}{H}\sum\limits_{h \in H}{L_h}$, respectively. Therefore, the peak to average in load demand for charging period is defined as follows:

% \begin{equation}
%     PAR = \frac{H \max_{h \in \mathcal{H}}{L_h}}{\sum\limits_{h \in H}{L_h}}.
% \end{equation}


\subsection{EV Network Centralized Minimization}
Considering the system model provided in Fig.~\ref{System Model}, the goal of an efficient EV charging controller can be twofold. Firstly, it aims to minimize the PAR to mitigate the risk of transformer overload during peak demand hours. Secondly, it aims to reduce the overall energy cost incurred by all end-users within the network. Our numerical results demonstrate that achieving goal one is a consequence of accomplishing goal two. Therefore, the formulation of the EV charging controller for minimizing the overall network cost can be as follows:

\begin{equation}\label{network_cost}
    \min_{i \in \mathscr{V}} & \sum\limits_{h=1}^{H} \mathbf{C}_h( \sum\limits_{i \in \mathscr{V}}{l_i^h}),
\end{equation}
where $\mathbf{C}_h$ denotes the network overall cost function at time step $h$.
Equation~\eqref{network_cost} can be easily solved in a centralized fashion, but solving it this way requires a centralized controller that has access to the information of all users, which makes the centralized node vulnerable to attackers. To address this issue, it is more advantageous to define a distributed control approach, where the smart meters use their charging control functionality with minimum information exchange among the smart meters and energy source. In particular, the goal is to let each smart meter, with its EV charging optimizer, control the EV charging rate connected to it, according to the local information of the users such as arrival/departure time, EV battery level, and expected battery level. 

\subsection{EV Network Decentralized Optimization}
To define a distributed solution for the problem in~\eqref{network_cost}, let define $b_{n}^h$ as billing amount in dollars to be charged to the user $n$ by the utility at time slot $h$. At any given time, users are charged proportional to their total energy demand. This means:
\begin{equation}\label{ProportionalDemand}
    \frac{b_{n}^h}{b_{m}^h} = \frac{l_{n}^h}{l_{m}^h}.
\end{equation}

Using~\eqref{ProportionalDemand} for the total cost of the network from user $n$ perspective at any given time, we have:

\begin{equation}\label{extended_proportionalDemand}
    \sum\limits_{n \in \mathscr{V}}{b_{n}^h} = \sum\limits_{n \in \mathscr{V}}{\frac{{b_{m}^h} \times l_{n}^h}{l_{m}^h}} = \frac{b_{m}^h}{l_{m}^h}\sum\limits_{n \in \mathscr{\mathscr{V}}}{l_{n}^h}.
\end{equation}

Together from \eqref{network_cost}, \eqref{ProportionalDemand}, and \eqref{extended_proportionalDemand} for each user we have:

\begin{align}\label{billing}
    b_{m}^h = \frac{l_{m}^h}{\sum\limits_{n \in \mathscr{V}}{l_{n}^h}}{\sum\limits_{n \in \mathscr{V}}{b_{n}^h}} = \frac{\kappa \times {l_{m}^h}}{\sum\limits_{n \in \mathscr{V}}{l_{n}^h}}{( \mathbf{C}_h( \sum\limits_{n \in \mathscr{V}}{l_n^h}))} =
    \nonumber \\
    \frac{\kappa \times {l_{m}^h}}{\sum\limits_{n \in \mathscr{V}}{l_{n}^h}}{( \mathbf{C}_h( {l_n^h}} + \sum\limits_{q \in \mathscr{V} \char`\\\{n\}}{l_{q}^h})),
\end{align}
where $\kappa$ is a constant coefficient. Equation \eqref{billing} illustrates that at any given time, the cost of the user $m$ not only depends on the local total consumption of the user $m$ ($l_m^h$), but also depends on other users' total consumption ($\sum\limits_{n \in \mathscr{V}}{l_n^h}$). 
Therefore, in distributed fashion, each agent aims to minimize its cost function as follows:
\begin{align}\label{NetwrokOptimization}
    \min_{l_{i}^h \in \mathcal{X}_i}
    \begin{aligned}[t]
      &\frac{\kappa \times {l_{i}^h}}{\sum\limits_{n \in \mathscr{V}}{l_{n}^h}}{( \mathbf{C}_h( {l_{i}^h}} + \sum\limits_{q \in \mathscr{V} \char`\\\{n\}}{l_{q}^h}))
   \end{aligned}
\end{align}
Thus, the user $i$ can solve the problem in~\eqref{NetwrokOptimization} as long as it knows the total EV consumption of other users. It is important to note that user $i$ does not require the detail information of the EV consumption of other users within the network. Knowing the overall EV consumption of the network is enough. This problem has been solved in~\cite{mohsenian2010autonomous} using game-theory with two assumptions: (1) End-users are charged proportional to their energy usage, which is unsuitable when dynamic pricing is implemented. (2) The daily energy consumption of all appliances including EV should be predetermined. The author in~\cite{yan2022cooperative}, solved this problem by relaxing these two assumption, but they assume that  each EV is capable of observing the total network demand at any given time.
Nevertheless, in order to maintain privacy, it is not appropriate to share this information among users. Additionally, this is not information that can be accessed by users in the real world. Thus, how agent $i$ can solve the problem in \ref{NetwrokOptimization} locally without the knowledge of other users EV consumption?


